Multiscaling in Hall-Magnetohydrodynamic Turbulence: Insights from a Shell Model

We show that a shell-model version of the three-dimensional Hall-magnetohydrodynamic (3D Hall-MHD) equations provides a natural theoretical model for investigating the multiscaling behaviors of velocity and magnetic structure functions. We carry out extensive numerical studies of this shell model, obtain the scaling exponents for its structure functions, in both the low-$k$ and high-$k$ power-law ranges of 3D Hall-MHD, and find that the extended-self-similarity (ESS) procedure is helpful in extracting the multiscaling nature of structure functions in the high-$k$ regime, which otherwise appears to display simple scaling. Our results shed light on intriguing solar-wind measurements.

==> 10pt.rtx.tex <==
%%
%% This is file `10pt.rtx',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% revtex4.dtx  (with options: `10pt')
%% 
%% This file is part of the APS files in the REVTeX 4 distribution.
%% For the version number, search on the string 
%% Original version by David Carlisle
%% Modified by Arthur Ogawa (mailto:ogawa@teleport.com)
%% 
%% Copyright (c) 1999 The American Physical Society.
%% http://publish.aps.org/revtex4/
%% mailto:revtex4@aps.org
%% 
%% See the REVTeX 4 README file for restrictions and more information.
%% 
\ProvidesFile{10pt.rtx}
          [2001/08/03 v4.0 (http://publish.aps.org/revtex4/ for documentation)]%FileInfo
\def\normalsize{%
   \@setfontsize\normalsize\@xpt{11.5}%
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \belowdisplayskip \abovedisplayskip
   \abovedisplayshortskip  \abovedisplayskip
   \belowdisplayshortskip \abovedisplayskip
   \let\@listi\@listI
}%
\def\small{%
  \@setfontsize\small\@ixpt{10.5}%
  \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
  \belowdisplayskip \abovedisplayskip
  \abovedisplayshortskip \z@ \@plus2\p@
  \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
  \def\@listi{%
    \leftmargin\leftmargini
    \topsep 4\p@ \@plus2\p@ \@minus2\p@
    \parsep 2\p@ \@plus\p@ \@minus\p@
    \itemsep \parsep
  }%
}%
\def\footnotesize{%
  \@setfontsize\footnotesize\@viiipt{9.5pt}%
  \abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
  \belowdisplayskip \abovedisplayskip
  \abovedisplayshortskip \z@ \@plus\p@
  \belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
  \def\@listi{%
    \leftmargin\leftmargini
    \topsep 3\p@ \@plus\p@ \@minus\p@
    \parsep 2\p@ \@plus\p@ \@minus\p@
    \itemsep \parsep
  }%
}%
\def\scriptsize{%
 \@setfontsize\scriptsize\@viipt\@viiipt
}%
\def\tiny{%
 \@setfontsize\tiny\@vpt\@vipt
}%
\def\large{%
 \@setfontsize\large\@xiipt{14pt}%
}%
\def\Large{%
 \@setfontsize\Large\@xivpt{18pt}%
}%
\def\LARGE{%
 \@setfontsize\LARGE\@xviipt{22pt}%
}%
\def\huge{%
 \@setfontsize\huge\@xxpt{25pt}%
}%
\def\Huge{%
 \@setfontsize\Huge\@xxvpt{30pt}%
}%
 \@ifxundefined\twoside@sw{\@booleanfalse\twoside@sw}{}%
 \twoside@sw{%
    \oddsidemargin  -20pt
    \evensidemargin -20pt
    \marginparwidth 107pt
 }{%
    \oddsidemargin  -.25in
    \evensidemargin -.25in
    \marginparwidth 30pt
 }%
\marginparsep 6pt
\topmargin -61pt
\headheight 25pt
\headsep 16pt
\topskip 10pt
\footskip 30pt
 \textheight = 56pc
\textwidth42.5pc
\columnsep 1.5pc
\columnseprule 0pt
\footnotesep 1pt
\skip\footins 39pt plus 4pt minus 2pt
\def\footnoterule{\kern-19pt\hrule width.5in\kern18.6pt\relax}%
\floatsep 12pt plus 2pt minus 2pt
\textfloatsep 20pt plus 2pt minus 4pt
\intextsep 12pt plus 2pt minus 2pt
\dblfloatsep 12pt plus 2pt minus 2pt
\dbltextfloatsep 20pt plus 2pt minus 4pt
\@fptop 0pt plus 1fil
\@fpsep 8pt plus 2fil
\@fpbot 0pt plus 1fil
\@dblfptop 0pt plus 1fil
\@dblfpsep 8pt plus 2fil
\@dblfpbot 0pt plus 1fil
\marginparpush 5pt
\parskip 0pt plus 1pt
\parindent 10pt
\emergencystretch8\p@
\partopsep 2pt plus 1pt minus 1pt
\leftmargini 25pt
\leftmarginii 22pt
\leftmarginiii 18.7pt
\leftmarginiv 17pt
\leftmarginv 10pt
\leftmarginvi 10pt
\def\@listI{%
  \leftmargin\leftmargini
  \parsep 4\p@ plus2\p@ minus\p@
  \topsep 8\p@ plus2\p@ minus4\p@
  \itemsep 4\p@ plus2\p@ minus\p@
}%
\labelsep 4pt
\def\@listii{%
  \leftmargin\leftmarginii
  \labelwidth\leftmarginii
  \advance\labelwidth-\labelsep
  \topsep 4\p@ plus2\p@ minus\p@
  \parsep 2\p@ plus\p@ minus\p@
  \itemsep \parsep
}%
\def\@listiii{%
  \leftmargin\leftmarginiii
  \labelwidth\leftmarginiii
  \advance\labelwidth-\labelsep
  \topsep 2\p@ plus\p@ minus\p@
  \parsep \z@
  \partopsep \p@ plus\z@ minus\p@
  \itemsep \topsep
}%
\def\@listiv{%
  \leftmargin\leftmarginiv
  \labelwidth\leftmarginiv
  \advance\labelwidth-\labelsep
}%
\def\@listv{%
  \leftmargin\leftmarginv
  \labelwidth\leftmarginv
  \advance\labelwidth-\labelsep
}%
\def\@listvi{%
  \leftmargin\leftmarginvi
  \labelwidth\leftmarginvi
  \advance\labelwidth-\labelsep
}%
\endinput
%%
%% End of file `10pt.rtx'.


==> aps.rtx.tex <==
	%%
	%% This is file `aps.rtx',
	%% generated with the docstrip utility.
	%%
	%% The original source files were:
	%%
	%% revtex4.dtx  (with options: `aps')
	%%
	%% This file is part of the APS files in the REVTeX 4 distribution.
	%% For the version number, search on the string
	%% Original version by David Carlisle
	%% Modified by Arthur Ogawa (mailto:ogawa@teleport.com)
	%%
	%% Copyright (c) 1999 The American Physical Society.
	%% http://publish.aps.org/revtex4/
	%% mailto:revtex4@aps.org
	%%
	%% See the REVTeX 4 README file for restrictions and more information.
	%%
	\NeedsTeXFormat{LaTeX2e}[1996/12/01]
	\ProvidesFile{aps.rtx}
	          [2001/08/03 v4.0 (http://publish.aps.org/revtex4/ for documentation)]%FileInfo
	\ifx\undefined\substyle@ext
	 \def\@tempa{%
	  \endinput
	  \GenericWarning{I must be read in by REVTeX! (Bailing out)}%
	 }%
	 \expandafter\else
	  \def\@tempa{}%
	 \expandafter\fi\@tempa
	\def\ao{Appl.\  Opt.\ }
	\def\ap{Appl.\  Phys.\ }
	\def\apl{Appl.\ Phys.\ Lett.\ }
	\def\apj{Astrophys.\ J.\ }
	\def\bell{Bell Syst.\ Tech.\ J.\ }
	\def\jqe{IEEE J.\ Quantum Electron.\ }
	\def\assp{IEEE Trans.\ Acoust.\ Speech Signal Process.\ }
	\def\aprop{IEEE Trans.\ Antennas Propag.\ }
	\def\mtt{IEEE Trans.\ Microwave Theory Tech.\ }
	\def\iovs{Invest.\ Ophthalmol.\ Vis.\ Sci.\ }
	\def\jcp{J.\ Chem.\ Phys.\ }
	\def\jmo{J.\ Mod.\ Opt.\ }
	\def\josa{J.\ Opt.\ Soc.\ Am.\ }
	\def\josaa{J.\ Opt.\ Soc.\ Am.\ A }
	\def\josab{J.\ Opt.\ Soc.\ Am.\ B }
	\def\jpp{J.\ Phys.\ (Paris) }
	\def\nat{Nature (London) }
	\def\oc{Opt.\ Commun.\ }
	\def\ol{Opt.\ Lett.\ }
	\def\pl{Phys.\ Lett.\ }
	\def\pra{Phys.\ Rev.\ A }
	\def\prb{Phys.\ Rev.\ B }
	\def\prc{Phys.\ Rev.\ C }
	\def\prd{Phys.\ Rev.\ D }
	\def\pre{Phys.\ Rev.\ E }
	\def\prl{Phys.\ Rev.\ Lett.\ }
	\def\rmp{Rev.\ Mod.\ Phys.\ }
	\def\pspie{Proc.\ Soc.\ Photo-Opt.\ Instrum.\ Eng.\ }
	\def\sjqe{Sov.\ J.\ Quantum Electron.\ }
	\def\vr{Vision Res.\ }
	\def\@fnsymbol#1{%
	 \ensuremath{%
	  \ifcase#1\or
	   *\or                        \dagger                   \or
	   \ddagger                \or \mathsection              \or
	   \mathparagraph\or
	   **\or                       \dagger\dagger            \or
	   \ddagger\ddagger        \or \mathsection \mathsection \or
	   \mathparagraph\mathparagraph\or
	   *{*}*\ignorespaces      \or \dagger\dagger\dagger     \or
	   \ddagger\ddagger\ddagger\or \mathsection \mathsection \mathsection \or
	   \mathparagraph\mathparagraph\mathparagraph\or
	  \else
	   \@ctrerr
	  \fi
	 }%
	}%
	\renewenvironment{titlepage}{%
	  \let\wastwocol@sw\twocolumn@sw
	  \onecolumngrid
	  \newpage
	  \thispagestyle{titlepage}%
	  \c@page\z@% article sets this to one not zero???
	}{%
	  \wastwocol@sw{\twocolumngrid}{\newpage}%
	}%
	\def\frontmatter@abstractheading{%
	 \preprintsty@sw{%
	  \begingroup
	   \centering\large
	   \abstractname
	   \par
	  \endgroup
	 }{}%
	}%
	\def\frontmatter@abstractwidth{400\p@}%
	\def\frontmatter@abstractfont{%
	 \small
	 \parindent1em\relax
	 \adjust@abstractwidth
	}%
	\def\adjust@abstractwidth{%
	 \dimen@\textwidth\advance\dimen@-\frontmatter@abstractwidth
	 \divide\dimen@\tw@
	 \galley@sw{%
	  \advance\rightskip\tw@\dimen@
	 }{%
	  \advance\leftskip\dimen@
	  \advance\rightskip\dimen@
	 }%
	}%
	\appdef\class@documenthook{%
	  \preprintsty@sw{%
	   \@ifxundefined\titlepage@sw{\@booleantrue\titlepage@sw}{}%
	   \def\frontmatter@abstractwidth{\textwidth}%
	   \def\frontmatter@affiliationfont{\it}%
	   \let\section\section@preprintsty
	   \let\subsection\subsection@preprintsty
	   \let\subsubsection\subsubsection@preprintsty
	  }{}%
	 }%
	\def\frontmatter@authorformat{%
	 \skip@\@flushglue
	 \@flushglue\z@ plus.3\hsize\relax
	 \centering
	 \advance\baselineskip\p@
	 \parskip11.5\p@\relax
	 \@flushglue\skip@
	}%
	\def\frontmatter@above@affilgroup{%
	}%
	\def\frontmatter@above@affiliation@script{%
	 \skip@\@flushglue
	 \@flushglue\z@ plus.3\hsize\relax
	 \centering
	 \@flushglue\skip@
	 \addvspace{3.5\p@}%
	}%
	\def\frontmatter@above@affiliation{%
	 \preprintsty@sw{}{%
	 }%
	}%
	\def\frontmatter@affiliationfont{%
	 \small\it
	}%
	\def\frontmatter@collaboration@above{%
	 \preprintsty@sw{%
	 }{%
	  \parskip1.5\p@\relax
	 }%
	}%
	\@ifxundefined\groupauthors@sw{%
	 \clo@groupedaddress
	}{}%
	\def\frontmatter@setup{%
	 \normalfont
	}%
	\def\frontmatter@title@above{\addvspace{6\p@}}%
	\def\frontmatter@title@format{\large\bfseries\centering\parskip\z@skip}%
	\def\frontmatter@title@below{}%
	\def\@author@parskip{3\p@}%
	\def\frontmatter@makefnmark{%
	 \@textsuperscript{%
	  \normalfont\@thefnmark
	 }%
	}%
	\def\frontmatter@authorbelow{%
	\addvspace{3\p@}%
	}%
	\def\frontmatter@RRAP@format{%
	  \small
	  \centering
	  \everypar{\hbox\bgroup(\@gobble@leavemode@uppercase}%
	  \def\par{\@ifvmode{}{\unskip)\egroup\@@par}}%
	}%
	\def\punct@RRAP{;\egroup\ \hbox\bgroup}%
	\def\@gobble@leavemode@uppercase#1#2{\expandafter\MakeTextUppercase}%
	\def\frontmatter@PACS@format{%
	   \addvspace{11\p@}%
	   \footnotesize
	   \adjust@abstractwidth
	   \parindent\z@
	   \parskip\z@skip
	   \samepage
	}%
	\def\frontmatter@keys@format{%
	   \footnotesize
	   \adjust@abstractwidth
	   \parindent\z@
	   \samepage
	}%
	\def\ps@titlepage{%
	  \def\@oddhead{%
	   \hfill
	   \produce@preprints\@preprint
	  }%
	  \let\@evenhead\@oddhead
	  \def\@oddfoot{%
	   \hb@xt@\z@{\byrevtex\hss}%
	   \hfil
	   \preprintsty@sw{\thepage}{}%
	   \quad\checkindate
	   \hfil
	  }%
	  \let\@evenfoot\@oddfoot
	}%
	\def\byrevtex{\byrevtex@sw{Typeset by REV\TeX}{}}%
	\def\produce@preprints#1{%
	 \preprint@sw{%
	  \vtop to \z@{%
	   \def\baselinestretch{1}%
	   \small
	   \let\preprint\preprint@count
	   \count@\z@#1\@ifnum{\count@>\tw@}{%
	    \hbox{%
	     \let\preprint\preprint@hlist
	     #1\setbox\z@\lastbox
	    }%
	   }{%
	    \let\preprint\preprint@cr
	    \halign{\hfil##\cr#1\crcr}%
	    \par
	    \vss
	   }%
	  }%
	 }{}%
	}%
	\def\preprint@cr#1{#1\cr}%
	\def\preprint@count#1{\advance\count@\@ne}%
	\def\preprint@hlist#1{#1\hbox{, }}%
	\def\@seccntformat#1{\csname the#1\endcsname.\quad}%
	\def\@hang@from#1#2#3{#1#2#3}%
	\def\section{%
	  \@startsection
	    {section}%
	    {1}%
	    {\z@}%
	    {0.8cm \@plus1ex \@minus .2ex}%
	    {0.5cm}%
	    {%
	      \normalfont\small\bfseries
	      \centering
	    }%
	}%
	\def\@hangfrom@section#1#2#3{\@hangfrom{#1#2}\MakeTextUppercase{#3}}%
	\def\subsection{%
	  \@startsection
	    {subsection}%
	    {2}%
	    {\z@}%
	    {.8cm \@plus1ex \@minus .2ex}%
	    {.5cm}%
	    {%
	     \normalfont\small\bfseries
	     \centering
	    }%
	}%
	\def\subsubsection{%
	  \@startsection
	    {subsubsection}%
	    {3}%
	    {\z@}%
	    {.8cm \@plus1ex \@minus .2ex}%
	    {.5cm}%
	    {%
	     \normalfont\small\itshape
	     \centering
	    }%
	}%
	\def\paragraph{%
	  \@startsection
	    {paragraph}%
	    {4}%
	    {\parindent}%
	    {\z@}%
	    {-1em}%
	    {\normalfont\normalsize\itshape}%
	}%
	\def\subparagraph{%
	  \@startsection
	    {subparagraph}%
	    {5}%
	    {\parindent}%
	    {3.25ex \@plus1ex \@minus .2ex}%
	    {-1em}%
	    {\normalfont\normalsize\bfseries}%
	}%
	\def\section@preprintsty{%
	  \@startsection
	    {section}%
	    {1}%
	    {\z@}%
	    {0.8cm \@plus1ex \@minus .2ex}%
	    {0.5cm}%
	    {%
	      \normalfont\small\bfseries
	    }%
	}%
	\def\subsection@preprintsty{%
	  \@startsection
	    {subsection}%
	    {2}%
	    {\z@}%
	    {.8cm \@plus1ex \@minus .2ex}%
	    {.5cm}%
	    {%
	     \normalfont\small\bfseries
	    }%
	}%
	\def\subsubsection@preprintsty{%
	  \@startsection
	    {subsubsection}%
	    {3}%
	    {\z@}%
	    {.8cm \@plus1ex \@minus .2ex}%
	    {.5cm}%
	    {%
	     \normalfont\small\itshape
	    }%
	}%
	 \@ifxundefined\frontmatter@footnote@produce{%
	  \let\frontmatter@footnote@produce\frontmatter@footnote@produce@endnote
	 }{}%
	\def\@pnumwidth{1.55em}
	\def\@tocrmarg {2.55em}
	\def\@dotsep{4.5pt}
	\setcounter{tocdepth}{3}
	\def\tableofcontents{%
	 \addtocontents{toc}{\string\tocdepth@munge}%
	 \print@toc{toc}%
	 \addtocontents{toc}{\string\tocdepth@restore}%
	}%
	\def\tocdepth@munge{%
	  \let\l@section@saved\l@section
	  \let\l@section\@gobble@tw@
	}%
	\def\@gobble@tw@#1#2{}%
	\def\tocdepth@restore{%
	  \let\l@section\l@section@saved
	}%
	\def\l@part#1#2{\addpenalty{\@secpenalty}%
	 \begingroup
	  \set@tocdim@pagenum{#2}%
	  \parindent \z@
	  \rightskip\tocleft@pagenum plus 1fil\relax
	  \skip@\parfillskip\parfillskip\z@
	  \addvspace{2.25em plus\p@}%
	  \large \bf %
	  \leavevmode\ignorespaces#1\unskip\nobreak\hskip\skip@
	  \hb@xt@\rightskip{\hfil\unhbox\z@}\hskip-\rightskip\hskip\z@skip
	  \par
	  \nobreak %
	 \endgroup
	}%
	\def\tocleft@{\z@}%
	\def\tocdim@min{5\p@}%
	\def\l@section{%
	 \l@@sections{}{section}% Implicit #3#4
	}%
	\def\l@f@section{%
	 \addpenalty{\@secpenalty}%
	 \addvspace{1.0em plus\p@}%
	 \bf
	}%
	\def\l@subsection{%
	 \l@@sections{section}{subsection}% Implicit #3#4
	}%
	\def\l@subsubsection{%
	 \l@@sections{subsection}{subsubsection}% Implicit #3#4
	}%
	\def\l@paragraph#1#2{}%
	\def\l@subparagraph#1#2{}%
	\let\toc@pre\toc@pre@auto
	\let\toc@post\toc@post@auto
	\def\listoffigures{\print@toc{lof}}%
	\def\l@figure{\@dottedtocline{1}{1.5em}{2.3em}}
	\def\listoftables{\print@toc{lot}}%
	\let\l@table\l@figure
	\appdef\class@documenthook{%
	 \@ifxundefined\raggedcolumn@sw{\@booleantrue\raggedcolumn@sw}{}%
	 \raggedcolumn@sw{\raggedbottom}{\flushbottom}%
	}%
	\def\tableft@skip@float{\z@ plus\hsize}%
	\def\tabmid@skip@float{\@flushglue}%
	\def\tabright@skip@float{\z@ plus\hsize}%
	\def\array@row@pre@float{\hline\hline\noalign{\vskip\doublerulesep}}%
	\def\array@row@pst@float{\noalign{\vskip\doublerulesep}\hline\hline}%
	\def\@makefntext#1{%
	 \def\baselinestretch{1}%
	 \reset@font
	 \footnotesize
	 \leftskip1em
	 \parindent1em
	 \noindent\nobreak\hskip-\leftskip
	 \hb@xt@\leftskip{%
	  \Hy@raisedlink{\hyper@anchorstart{footnote@\the\c@footnote}\hyper@anchorend}%
	  \hss\@makefnmark\
	 }%
	 #1%
	 \par
	}%
	\prepdef\appendix{%
	 \par
	 \let\@hangfrom@section\@hangfrom@appendix
	 \let\@hangfroms@section\@hangfroms@appendix
	 \let\@sectioncntformat\@appendixcntformat
	}%
	\def\@hangfrom@appendix#1#2#3{%
	 #1%
	 \@if@empty{#2}{%
	  \MakeTextUppercase{#3}%
	 }{%
	  #2\@if@empty{#3}{}{:\ \MakeTextUppercase{#3}}%
	 }%
	}%
	\def\@hangfroms@appendix#1#2{%
	 #1\MakeTextUppercase{#2}%
	}%
	\def\@appendixcntformat#1{\appendixname\ \csname the#1\endcsname}%
	\def\appendixesname{APPENDICES}%
	\def\appendixname{APPENDIX}%
	 \bibpunct{[}{]}{,}{n}{}{,}%
	 \def\bibsection{%
	  \par
	  \onecolumngrid@push
	  \begingroup
	   \baselineskip26\p@
	   \bib@device{\textwidth}{245.5\p@}%
	 \endgroup
	  \nobreak\@nobreaktrue
	  \addvspace{19\p@}%
	  \par
	  \onecolumngrid@pop
	 }%
	\def\bib@device#1#2{%
	\hb@xt@#1{%
	 \hfil
	 \phantomsection
	  \addcontentsline {toc}{section}{\protect\numberline{}\refname}%
	 \hb@xt@#2{%
	  \skip@\z@\@plus-1fil\relax
	                        \leaders\hrule height.25 \p@ depth.25 \p@ \hskip\z@\@plus1fil
	\hskip\skip@
	\hskip\z@\@plus0.125fil\leaders\hrule height.375\p@ depth.375\p@ \hskip\z@\@plus0.75fil \hskip\z@\@plus0.125fil
	\hskip\skip@
	\hskip\z@\@plus0.25 fil\leaders\hrule height.5  \p@ depth.5  \p@ \hskip\z@\@plus0.5 fil \hskip\z@\@plus0.25 fil
	\hskip\skip@
	\hskip\z@\@plus0.375fil\leaders\hrule height.625\p@ depth.625\p@ \hskip\z@\@plus0.25fil \hskip\z@\@plus0.375fil
	 }%
	\hfil
	}%
	}%
	\let\bibpreamble\@empty
	\bibsep\z@\relax
	\def\newblock{\ }%
	 \def\bibfont{%
	  \small
	 }%
	\newenvironment{theindex}{%
	 \columnseprule \z@
	 \columnsep 35\p@
	 \c@secnumdepth-\maxdimen
	 \onecolumngrid@push
	 \section{\indexname}%
	 \thispagestyle{plain}%
	 \parindent\z@
	 \parskip\z@ plus.3\p@\relax
	 \let\item\@idxitem
	 \onecolumngrid@pop
	}{%
	}%
	\def\@idxitem{\par\hangindent 40\p@}
	\def\subitem{\par\hangindent 40\p@ \hspace*{20\p@}}
	\def\subsubitem{\par\hangindent 40\p@ \hspace*{30\p@}}
	\def\indexspace{\par \vskip 10\p@ plus5\p@ minus3\p@\relax}
	\def\journal@pra{pra}%
	\def\journal@prb{prb}%
	\def\journal@prc{prc}%
	\def\journal@prd{prd}%
	\def\journal@pre{pre}%
	\def\journal@prl{prl}%
	\def\journal@prstab{prstab}%
	\def\journal@rmp{rmp}%
	\@ifx{\@journal\journal@pra}{%
	}{}%
	\@ifx{\@journal\journal@prb}{%
	 \@ifxundefined\bibnotes@sw{\@booleantrue\bibnotes@sw}{}%
	 \bibpunct{}{}{,}{s}{}{\textsuperscript{,}}%
	 \def\@onlinecite#1{\begingroup\let\@cite\NAT@citenum\citealp{#1}\endgroup}%
	 \appdef\class@documenthook{%
	  \@ifxundefined\place@bibnumber{%
	   \let\place@bibnumber\place@bibnumber@sup
	  }{}%
	 }%
	}{}%
	\@ifx{\@journal\journal@prc}{%
	}{}%
	\@ifx{\@journal\journal@prd}{%
	}{}%
	\@ifx{\@journal\journal@pre}{%
	}{}%
	\@ifx{\@journal\journal@prl}{%
	 \@ifxundefined\bibnotes@sw{\@booleantrue\bibnotes@sw}{}%
	 \@booleanfalse\acknowledgments@sw
	 \def\bibsection{%
	  \par
	  \begingroup
	   \baselineskip26\p@
	   \bib@device{\hsize}{72\p@}%
	 \endgroup
	  \nobreak\@nobreaktrue
	  \addvspace{19\p@}%
	 }%
	 \@ifxundefined\lengthcheck@sw{\@booleanfalse\lengthcheck@sw}{}%
	  \lengthcheck@sw{%
	   \RequirePackage{times}%
	  }{%
	  }%
	 \c@secnumdepth=-\maxdimen
	 \appdef\set@typesize@hook{%
	  \@ifnum{\@pointsize=10\relax}{%
	   \lengthcheck@sw{%
	    \def\large{%
	     \@setfontsize\large{12.5}{14\p@}%
	    }%
	    \def\normalsize{%
	     \@setfontsize\normalsize{10.5}\@xiipt
	     \abovedisplayskip 6\p@ \@plus6\p@ \@minus5\p@
	     \belowdisplayskip \abovedisplayskip
	     \abovedisplayshortskip  \abovedisplayskip
	     \belowdisplayshortskip \abovedisplayskip
	     \let\@listi\@listI
	    }%
	    \def\small{%
	     \@setfontsize\small{9.5}\@xipt
	     \abovedisplayskip 5\p@ \@plus5\p@ \@minus4\p@
	     \belowdisplayskip \abovedisplayskip
	     \abovedisplayshortskip  \abovedisplayskip
	     \belowdisplayshortskip \abovedisplayskip
	     \let\@listi\@listI
	    }%
	    \DeclareMathSizes{12.5}{12.5}{9}{6}%
	    \DeclareMathSizes{10.5}{10.5}{7.5}{5}%
	    \DeclareMathSizes{9.5}{9.5}{7.0}{5}%
	   }{%
	    \def\normalsize{%
	     \@setfontsize\normalsize\@xpt\@xiipt
	     \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
	     \belowdisplayskip \abovedisplayskip
	     \abovedisplayshortskip  \abovedisplayskip
	     \belowdisplayshortskip \abovedisplayskip
	     \let\@listi\@listI
	    }%
	   }%
	  }{}%
	 }%
	  \@ifnum{\@pointsize=10\relax}{%
	   \textheight = 694.0\p@
	  }{}%
	}{}%
	\@ifx{\@journal\journal@prstab}{%
	}{}%
	\@ifx{\@journal\journal@rmp}{\input{\@journal\substyle@ext}}{}%
	\@ifxundefined\footinbib@sw{\@booleantrue\footinbib@sw}{}%
	\appdef\class@documenthook{%
	 \@ifxundefined\place@bibnumber{%
	  \let\place@bibnumber\place@bibnumber@inl
	 }{}%
	 \@ifxundefined\@bibstyle{%
	  \def\@bibstyle{apsrev}%
	 }{}%
	}%
	\endinput
	%%
	%% End of file `aps.rtx'.

